FAST drift scan survey for HI intensity mapping: I. preliminary data analysis

This work presents the initial results of the drift-scan observation for the neutral hydrogen (HI) intensity mapping survey with the Five-hundred-meter Aperture Spherical radio Telescope (FAST). The data analyzed in this work were collected in night observations from 2019 through 2021. The primary findings are based on 28 hours of drift-scan observation carried out over seven nights in 2021, which covers $60\,{\rm deg}^2$ sky area. Our main findings are: (i) Our calibration strategy can successfully correct both the temporal and bandpass gain variation over the $4$-hour drift-scan observation. (ii) The continuum maps of the surveyed region are made with frequency resolution of $28$ kHz and pixel area of $2.95\,{\rm arcmin}^2$. The pixel noise levels of the continuum maps are slightly higher than the forecast assuming $T_{\rm sys}=20\,{\rm K}$, which are $36.0$ mK (for 10.0 s integration time) at the $1050$--$1150$ MHz band, and $25.9$ mK (for 16.7 s integration time) at the $1323$--$1450$ MHz band, respectively. (iii) The flux-weighted differential number count is consistent with the NRAO-VLA Sky Survey (NVSS) catalog down to the confusion limit $\sim7\,{\rm mJy}/{\rm beam}^{-1}$. (iv) The continuum flux measurements of the sources are consistent with that found in the literature. The difference in the flux measurement of $81$ isolated NVSS sources is about $6.3\%$. Our research offers a systematic analysis for the FAST HI intensity mapping drift-scan survey and serves as a helpful resource for further cosmology and associated galaxies sciences with the FAST drift-scan survey.

==> FAST HIMGS 20230511 arxiv/results_todsource_ap1p5.tex <==
\begin{tabular}{ccrrr | ccrrr} \hline\hline
 RA (J2000) & Dec (J2000) & $S_{\rm NVSS}$ & $S_{\rm FAST}$ & Correction   & RA (J2000) & Dec (J2000) & $S_{\rm NVSS}$ & $S_{\rm FAST}$ & Correction \\
            &             & $[{\rm mJy}] $ & $[{\rm mJy}] $ & [$\%$] &            &             & $[{\rm mJy}] $ & $[{\rm mJy}] $ & [$\%$] \\\hline
$09\overset{\rm h}{} 03\overset{\rm m}{} 11\overset{{\rm s}}{.}67$ & $+26\overset{\circ}{} 09\overset{\prime}{} 40\overset{{\prime\prime}}{.}28$ & $ 195.87$ & $ 184.04 \pm  3.88$ &$  13.35$ &$09\overset{\rm h}{} 42\overset{\rm m}{} 36\overset{{\rm s}}{.}39$ & $+26\overset{\circ}{} 10\overset{\prime}{} 15\overset{{\prime\prime}}{.}27$ & $  35.09$ & $  27.41 \pm  0.90$ &$  13.08$ \\
$10\overset{\rm h}{} 18\overset{\rm m}{} 07\overset{{\rm s}}{.}13$ & $+26\overset{\circ}{} 09\overset{\prime}{} 42\overset{{\prime\prime}}{.}51$ & $ 180.38$ & $ 177.66 \pm  3.80$ &$  13.99$ &$09\overset{\rm h}{} 26\overset{\rm m}{} 00\overset{{\rm s}}{.}53$ & $+25\overset{\circ}{} 59\overset{\prime}{} 53\overset{{\prime\prime}}{.}30$ & $ 113.56$ & $ 115.60 \pm  2.97$ &$   9.24$ \\
$10\overset{\rm h}{} 57\overset{\rm m}{} 23\overset{{\rm s}}{.}15$ & $+26\overset{\circ}{} 01\overset{\prime}{} 30\overset{{\prime\prime}}{.}18$ & $ 186.74$ & $ 188.67 \pm  4.89$ &$   4.92$ &$11\overset{\rm h}{} 34\overset{\rm m}{} 02\overset{{\rm s}}{.}19$ & $+26\overset{\circ}{} 32\overset{\prime}{} 24\overset{{\prime\prime}}{.}54$ & $  15.62$ & $  13.75 \pm  0.39$ &$  13.94$ \\
$12\overset{\rm h}{} 38\overset{\rm m}{} 23\overset{{\rm s}}{.}54$ & $+26\overset{\circ}{} 33\overset{\prime}{} 46\overset{{\prime\prime}}{.}43$ & $ 104.30$ & $  97.35 \pm  3.34$ &$  -0.27$ &$12\overset{\rm h}{} 39\overset{\rm m}{} 52\overset{{\rm s}}{.}76$ & $+26\overset{\circ}{} 32\overset{\prime}{} 46\overset{{\prime\prime}}{.}57$ & $  49.14$ & $  45.11 \pm  1.52$ &$  10.42$ \\
$12\overset{\rm h}{} 48\overset{\rm m}{} 41\overset{{\rm s}}{.}35$ & $+26\overset{\circ}{} 33\overset{\prime}{} 56\overset{{\prime\prime}}{.}48$ & $  74.42$ & $  70.56 \pm  2.54$ &$   1.94$ &$10\overset{\rm h}{} 13\overset{\rm m}{} 36\overset{{\rm s}}{.}86$ & $+26\overset{\circ}{} 52\overset{\prime}{} 06\overset{{\prime\prime}}{.}67$ & $ 157.57$ & $ 139.77 \pm  3.66$ &$   9.56$ \\
$10\overset{\rm h}{} 45\overset{\rm m}{} 57\overset{{\rm s}}{.}36$ & $+26\overset{\circ}{} 52\overset{\prime}{} 39\overset{{\prime\prime}}{.}93$ & $  56.87$ & $  46.13 \pm  1.41$ &$  12.77$ &$10\overset{\rm h}{} 46\overset{\rm m}{} 40\overset{{\rm s}}{.}38$ & $+26\overset{\circ}{} 54\overset{\prime}{} 15\overset{{\prime\prime}}{.}73$ & $ 163.09$ & $ 155.16 \pm  3.46$ &$  13.96$ \\
$09\overset{\rm h}{} 21\overset{\rm m}{} 58\overset{{\rm s}}{.}57$ & $+26\overset{\circ}{} 21\overset{\prime}{} 22\overset{{\prime\prime}}{.}60$ & $ 206.52$ & $ 211.16 \pm  5.83$ &$   1.16$ &$10\overset{\rm h}{} 16\overset{\rm m}{} 00\overset{{\rm s}}{.}82$ & $+26\overset{\circ}{} 22\overset{\prime}{} 00\overset{{\prime\prime}}{.}12$ & $  27.87$ & $  23.13 \pm  0.81$ &$   2.94$ \\
$10\overset{\rm h}{} 48\overset{\rm m}{} 28\overset{{\rm s}}{.}59$ & $+26\overset{\circ}{} 22\overset{\prime}{} 34\overset{{\prime\prime}}{.}89$ & $ 237.69$ & $ 244.67 \pm  6.13$ &$   0.52$ &$10\overset{\rm h}{} 52\overset{\rm m}{} 52\overset{{\rm s}}{.}26$ & $+26\overset{\circ}{} 22\overset{\prime}{} 16\overset{{\prime\prime}}{.}24$ & $ 105.61$ & $ 105.37 \pm  2.62$ &$   2.66$ \\
$09\overset{\rm h}{} 27\overset{\rm m}{} 45\overset{{\rm s}}{.}09$ & $+26\overset{\circ}{} 13\overset{\prime}{} 00\overset{{\prime\prime}}{.}51$ & $ 150.04$ & $ 146.74 \pm  3.36$ &$  13.82$ &$10\overset{\rm h}{} 40\overset{\rm m}{} 37\overset{{\rm s}}{.}59$ & $+26\overset{\circ}{} 13\overset{\prime}{} 24\overset{{\prime\prime}}{.}81$ & $  29.96$ & $  25.01 \pm  1.14$ &$  13.45$ \\
$10\overset{\rm h}{} 54\overset{\rm m}{} 56\overset{{\rm s}}{.}64$ & $+26\overset{\circ}{} 12\overset{\prime}{} 47\overset{{\prime\prime}}{.}26$ & $ 338.51$ & $ 337.11 \pm  7.16$ &$  12.35$ &$12\overset{\rm h}{} 11\overset{\rm m}{} 29\overset{{\rm s}}{.}70$ & $+26\overset{\circ}{} 14\overset{\prime}{} 50\overset{{\prime\prime}}{.}20$ & $  67.80$ & $  64.70 \pm  1.25$ &$  14.18$ \\
$09\overset{\rm h}{} 49\overset{\rm m}{} 06\overset{{\rm s}}{.}44$ & $+26\overset{\circ}{} 01\overset{\prime}{} 57\overset{{\prime\prime}}{.}71$ & $  20.78$ & $  11.63 \pm  0.87$ &$  15.45$ &$12\overset{\rm h}{} 57\overset{\rm m}{} 12\overset{{\rm s}}{.}52$ & $+26\overset{\circ}{} 01\overset{\prime}{} 40\overset{{\prime\prime}}{.}62$ & $  62.57$ & $  55.22 \pm  1.23$ &$   1.79$ \\
$09\overset{\rm h}{} 18\overset{\rm m}{} 56\overset{{\rm s}}{.}17$ & $+26\overset{\circ}{} 33\overset{\prime}{} 30\overset{{\prime\prime}}{.}99$ & $  20.90$ & $  18.22 \pm  0.82$ &$  22.58$ &$10\overset{\rm h}{} 39\overset{\rm m}{} 30\overset{{\rm s}}{.}97$ & $+26\overset{\circ}{} 33\overset{\prime}{} 03\overset{{\prime\prime}}{.}88$ & $ 143.48$ & $ 133.02 \pm  3.53$ &$   1.31$ \\
$10\overset{\rm h}{} 59\overset{\rm m}{} 07\overset{{\rm s}}{.}98$ & $+26\overset{\circ}{} 34\overset{\prime}{} 07\overset{{\prime\prime}}{.}50$ & $  56.83$ & $  55.56 \pm  1.47$ &$   6.01$ &$12\overset{\rm h}{} 36\overset{\rm m}{} 30\overset{{\rm s}}{.}59$ & $+26\overset{\circ}{} 35\overset{\prime}{} 19\overset{{\prime\prime}}{.}78$ & $ 564.07$ & $ 599.41 \pm 20.89$ &$  29.70$ \\
$11\overset{\rm h}{} 22\overset{\rm m}{} 04\overset{{\rm s}}{.}96$ & $+26\overset{\circ}{} 13\overset{\prime}{} 36\overset{{\prime\prime}}{.}73$ & $ 303.49$ & $ 300.70 \pm  5.84$ &$  12.37$ &$10\overset{\rm h}{} 22\overset{\rm m}{} 09\overset{{\rm s}}{.}14$ & $+26\overset{\circ}{} 23\overset{\prime}{} 13\overset{{\prime\prime}}{.}70$ & $ 161.25$ & $ 161.32 \pm  4.29$ &$   7.96$ \\
$10\overset{\rm h}{} 55\overset{\rm m}{} 47\overset{{\rm s}}{.}35$ & $+26\overset{\circ}{} 23\overset{\prime}{} 37\overset{{\prime\prime}}{.}82$ & $ 152.02$ & $ 150.63 \pm  3.38$ &$   6.00$ &$12\overset{\rm h}{} 05\overset{\rm m}{} 32\overset{{\rm s}}{.}86$ & $+26\overset{\circ}{} 25\overset{\prime}{} 40\overset{{\prime\prime}}{.}65$ & $ 278.72$ & $ 268.41 \pm  4.18$ &$  27.54$ \\
$11\overset{\rm h}{} 25\overset{\rm m}{} 00\overset{{\rm s}}{.}85$ & $+26\overset{\circ}{} 06\overset{\prime}{} 09\overset{{\prime\prime}}{.}32$ & $  56.43$ & $  46.94 \pm  1.60$ &$   5.32$ &$12\overset{\rm h}{} 19\overset{\rm m}{} 56\overset{{\rm s}}{.}37$ & $+26\overset{\circ}{} 07\overset{\prime}{} 04\overset{{\prime\prime}}{.}07$ & $ 109.12$ & $  62.21 \pm  2.72$ &$  10.48$ \\
$12\overset{\rm h}{} 21\overset{\rm m}{} 02\overset{{\rm s}}{.}00$ & $+26\overset{\circ}{} 08\overset{\prime}{} 45\overset{{\prime\prime}}{.}74$ & $ 199.08$ & $ 123.17 \pm  2.70$ &$   9.95$ &$09\overset{\rm h}{} 02\overset{\rm m}{} 54\overset{{\rm s}}{.}70$ & $+25\overset{\circ}{} 55\overset{\prime}{} 44\overset{{\prime\prime}}{.}83$ & $  19.08$ & $  21.38 \pm  1.02$ &$  19.49$ \\
$09\overset{\rm h}{} 16\overset{\rm m}{} 47\overset{{\rm s}}{.}38$ & $+25\overset{\circ}{} 54\overset{\prime}{} 16\overset{{\prime\prime}}{.}05$ & $  73.79$ & $  68.79 \pm  2.34$ &$   4.71$ &$09\overset{\rm h}{} 28\overset{\rm m}{} 53\overset{{\rm s}}{.}21$ & $+25\overset{\circ}{} 54\overset{\prime}{} 37\overset{{\prime\prime}}{.}90$ & $  69.09$ & $  68.43 \pm  2.45$ &$   9.84$ \\
$09\overset{\rm h}{} 33\overset{\rm m}{} 15\overset{{\rm s}}{.}67$ & $+25\overset{\circ}{} 55\overset{\prime}{} 00\overset{{\prime\prime}}{.}69$ & $  61.57$ & $  62.32 \pm  2.06$ &$  12.20$ &$09\overset{\rm h}{} 44\overset{\rm m}{} 42\overset{{\rm s}}{.}33$ & $+25\overset{\circ}{} 54\overset{\prime}{} 43\overset{{\prime\prime}}{.}55$ & $ 774.39$ & $ 771.98 \pm 19.53$ &$   7.81$ \\
$09\overset{\rm h}{} 45\overset{\rm m}{} 53\overset{{\rm s}}{.}28$ & $+25\overset{\circ}{} 56\overset{\prime}{} 08\overset{{\prime\prime}}{.}37$ & $  54.64$ & $  55.52 \pm  1.17$ &$  22.19$ &$11\overset{\rm h}{} 08\overset{\rm m}{} 38\overset{{\rm s}}{.}99$ & $+25\overset{\circ}{} 56\overset{\prime}{} 13\overset{{\prime\prime}}{.}45$ & $  88.49$ & $  98.64 \pm  2.68$ &$   5.22$ \\
$09\overset{\rm h}{} 40\overset{\rm m}{} 13\overset{{\rm s}}{.}47$ & $+26\overset{\circ}{} 26\overset{\prime}{} 56\overset{{\prime\prime}}{.}68$ & $ 124.22$ & $ 107.93 \pm  2.82$ &$   5.26$ &$12\overset{\rm h}{} 53\overset{\rm m}{} 02\overset{{\rm s}}{.}00$ & $+26\overset{\circ}{} 27\overset{\prime}{} 45\overset{{\prime\prime}}{.}97$ & $ 203.70$ & $ 166.13 \pm  7.02$ &$   2.76$ \\
$09\overset{\rm h}{} 18\overset{\rm m}{} 37\overset{{\rm s}}{.}49$ & $+26\overset{\circ}{} 50\overset{\prime}{} 41\overset{{\prime\prime}}{.}10$ & $ 105.95$ & $ 103.85 \pm  3.05$ &$   8.58$ &$10\overset{\rm h}{} 42\overset{\rm m}{} 43\overset{{\rm s}}{.}59$ & $+26\overset{\circ}{} 50\overset{\prime}{} 02\overset{{\prime\prime}}{.}25$ & $ 148.24$ & $ 151.05 \pm  3.48$ &$   6.64$ \\
$12\overset{\rm h}{} 04\overset{\rm m}{} 12\overset{{\rm s}}{.}95$ & $+26\overset{\circ}{} 50\overset{\prime}{} 58\overset{{\prime\prime}}{.}95$ & $ 417.72$ & $ 420.74 \pm  9.65$ &$  12.98$ &$12\overset{\rm h}{} 19\overset{\rm m}{} 46\overset{{\rm s}}{.}58$ & $+26\overset{\circ}{} 17\overset{\prime}{} 34\overset{{\prime\prime}}{.}40$ & $  29.46$ & $  17.75 \pm  0.92$ &$  17.36$ \\
$12\overset{\rm h}{} 20\overset{\rm m}{} 27\overset{{\rm s}}{.}95$ & $+26\overset{\circ}{} 19\overset{\prime}{} 03\overset{{\prime\prime}}{.}54$ & $  32.41$ & $  17.92 \pm  0.28$ &$  12.38$ &$09\overset{\rm h}{} 13\overset{\rm m}{} 27\overset{{\rm s}}{.}12$ & $+26\overset{\circ}{} 02\overset{\prime}{} 23\overset{{\prime\prime}}{.}13$ & $  67.04$ & $  61.94 \pm  1.10$ &$  30.81$ \\
$09\overset{\rm h}{} 17\overset{\rm m}{} 15\overset{{\rm s}}{.}57$ & $+26\overset{\circ}{} 03\overset{\prime}{} 40\overset{{\prime\prime}}{.}53$ & $  58.42$ & $  49.17 \pm  1.41$ &$   7.95$ &$09\overset{\rm h}{} 40\overset{\rm m}{} 14\overset{{\rm s}}{.}71$ & $+26\overset{\circ}{} 03\overset{\prime}{} 29\overset{{\prime\prime}}{.}91$ & $ 462.22$ & $ 457.43 \pm 13.37$ &$  21.65$ \\
$09\overset{\rm h}{} 41\overset{\rm m}{} 28\overset{{\rm s}}{.}66$ & $+26\overset{\circ}{} 04\overset{\prime}{} 02\overset{{\prime\prime}}{.}56$ & $  79.37$ & $  77.97 \pm  2.18$ &$   8.46$ &$10\overset{\rm h}{} 05\overset{\rm m}{} 15\overset{{\rm s}}{.}06$ & $+26\overset{\circ}{} 03\overset{\prime}{} 35\overset{{\prime\prime}}{.}99$ & $ 180.10$ & $ 165.31 \pm  3.55$ &$  23.18$ \\
$10\overset{\rm h}{} 24\overset{\rm m}{} 19\overset{{\rm s}}{.}44$ & $+26\overset{\circ}{} 05\overset{\prime}{} 10\overset{{\prime\prime}}{.}71$ & $  20.86$ & $  18.40 \pm  0.50$ &$   5.51$ &$12\overset{\rm h}{} 22\overset{\rm m}{} 01\overset{{\rm s}}{.}84$ & $+26\overset{\circ}{} 04\overset{\prime}{} 15\overset{{\prime\prime}}{.}09$ & $  60.17$ & $  32.34 \pm  0.98$ &$  28.94$ \\
$09\overset{\rm h}{} 30\overset{\rm m}{} 27\overset{{\rm s}}{.}63$ & $+25\overset{\circ}{} 52\overset{\prime}{} 54\overset{{\prime\prime}}{.}26$ & $  78.58$ & $  83.92 \pm  2.25$ &$  16.53$ &$09\overset{\rm h}{} 17\overset{\rm m}{} 17\overset{{\rm s}}{.}69$ & $+26\overset{\circ}{} 45\overset{\prime}{} 51\overset{{\prime\prime}}{.}73$ & $  22.46$ & $  21.96 \pm  0.73$ &$  14.87$ \\
$10\overset{\rm h}{} 35\overset{\rm m}{} 16\overset{{\rm s}}{.}54$ & $+26\overset{\circ}{} 15\overset{\prime}{} 16\overset{{\prime\prime}}{.}45$ & $ 388.16$ & $ 367.07 \pm  7.47$ &$   9.77$ &$12\overset{\rm h}{} 02\overset{\rm m}{} 55\overset{{\rm s}}{.}33$ & $+26\overset{\circ}{} 15\overset{\prime}{} 18\overset{{\prime\prime}}{.}79$ & $  51.15$ & $  39.83 \pm  1.00$ &$  13.88$ \\
$11\overset{\rm h}{} 34\overset{\rm m}{} 34\overset{{\rm s}}{.}12$ & $+26\overset{\circ}{} 52\overset{\prime}{} 50\overset{{\prime\prime}}{.}95$ & $ 108.72$ & $  99.49 \pm  2.50$ &$  14.70$ &$09\overset{\rm h}{} 05\overset{\rm m}{} 05\overset{{\rm s}}{.}60$ & $+26\overset{\circ}{} 11\overset{\prime}{} 23\overset{{\prime\prime}}{.}24$ & $ 207.10$ & $ 191.89 \pm  4.47$ &$  10.57$ \\
$10\overset{\rm h}{} 11\overset{\rm m}{} 06\overset{{\rm s}}{.}75$ & $+26\overset{\circ}{} 38\overset{\prime}{} 21\overset{{\prime\prime}}{.}01$ & $  33.34$ & $  27.02 \pm  1.47$ &$   9.53$ &$10\overset{\rm h}{} 19\overset{\rm m}{} 26\overset{{\rm s}}{.}26$ & $+26\overset{\circ}{} 38\overset{\prime}{} 58\overset{{\prime\prime}}{.}41$ & $ 117.41$ & $ 119.92 \pm  3.15$ &$  10.87$ \\
$10\overset{\rm h}{} 25\overset{\rm m}{} 08\overset{{\rm s}}{.}32$ & $+26\overset{\circ}{} 36\overset{\prime}{} 39\overset{{\prime\prime}}{.}24$ & $  14.53$ & $   8.41 \pm  1.04$ &$  17.35$ &$10\overset{\rm h}{} 31\overset{\rm m}{} 56\overset{{\rm s}}{.}02$ & $+26\overset{\circ}{} 38\overset{\prime}{} 20\overset{{\prime\prime}}{.}94$ & $  96.73$ & $  95.41 \pm  3.55$ &$   9.19$ \\
$10\overset{\rm h}{} 57\overset{\rm m}{} 24\overset{{\rm s}}{.}93$ & $+26\overset{\circ}{} 38\overset{\prime}{} 00\overset{{\prime\prime}}{.}02$ & $ 435.24$ & $ 420.13 \pm 14.35$ &$   4.35$ &$11\overset{\rm h}{} 25\overset{\rm m}{} 20\overset{{\rm s}}{.}26$ & $+26\overset{\circ}{} 38\overset{\prime}{} 02\overset{{\prime\prime}}{.}07$ & $  49.37$ & $  40.30 \pm  1.67$ &$   5.63$ \\
$09\overset{\rm h}{} 23\overset{\rm m}{} 43\overset{{\rm s}}{.}10$ & $+26\overset{\circ}{} 34\overset{\prime}{} 49\overset{{\prime\prime}}{.}94$ & $  41.15$ & $  38.81 \pm  1.30$ &$  34.81$ &$12\overset{\rm h}{} 42\overset{\rm m}{} 48\overset{{\rm s}}{.}21$ & $+25\overset{\circ}{} 58\overset{\prime}{} 40\overset{{\prime\prime}}{.}76$ & $ 308.33$ & $ 290.77 \pm  6.32$ &$  17.88$ \\
$11\overset{\rm h}{} 06\overset{\rm m}{} 08\overset{{\rm s}}{.}35$ & $+25\overset{\circ}{} 52\overset{\prime}{} 13\overset{{\prime\prime}}{.}04$ & $  38.26$ & $  39.91 \pm  1.97$ &$  10.67$ &$11\overset{\rm h}{} 27\overset{\rm m}{} 05\overset{{\rm s}}{.}77$ & $+25\overset{\circ}{} 50\overset{\prime}{} 55\overset{{\prime\prime}}{.}17$ & $ 117.51$ & $ 127.43 \pm  3.32$ &$   2.96$ \\
$12\overset{\rm h}{} 00\overset{\rm m}{} 05\overset{{\rm s}}{.}07$ & $+26\overset{\circ}{} 44\overset{\prime}{} 18\overset{{\prime\prime}}{.}34$ & $  34.49$ & $  40.04 \pm  1.21$ &$   6.54$ &$10\overset{\rm h}{} 33\overset{\rm m}{} 40\overset{{\rm s}}{.}04$ & $+26\overset{\circ}{} 42\overset{\prime}{} 57\overset{{\prime\prime}}{.}77$ & $  16.66$ & $  16.56 \pm  0.57$ &$  13.50$ \\
$10\overset{\rm h}{} 54\overset{\rm m}{} 40\overset{{\rm s}}{.}25$ & $+26\overset{\circ}{} 41\overset{\prime}{} 25\overset{{\prime\prime}}{.}69$ & $  63.90$ & $  59.84 \pm  1.59$ &$   7.20$ &$10\overset{\rm h}{} 14\overset{\rm m}{} 14\overset{{\rm s}}{.}85$ & $+25\overset{\circ}{} 52\overset{\prime}{} 00\overset{{\prime\prime}}{.}01$ & $  37.40$ & $  30.04 \pm  1.06$ &$  21.30$ \\
$09\overset{\rm h}{} 54\overset{\rm m}{} 39\overset{{\rm s}}{.}79$ & $+26\overset{\circ}{} 39\overset{\prime}{} 24\overset{{\prime\prime}}{.}55$ & $ 312.67$ & $ 302.08 \pm  5.82$ &$  13.77$ &$10\overset{\rm h}{} 39\overset{\rm m}{} 50\overset{{\rm s}}{.}71$ & $+27\overset{\circ}{} 01\overset{\prime}{} 48\overset{{\prime\prime}}{.}14$ & $  14.86$ & $  14.63 \pm  0.73$ &$   5.01$ \\
$12\overset{\rm h}{} 24\overset{\rm m}{} 21\overset{{\rm s}}{.}36$ & $+27\overset{\circ}{} 01\overset{\prime}{} 42\overset{{\prime\prime}}{.}20$ & $  97.89$ & $  95.13 \pm  2.15$ &$   7.08$ &$09\overset{\rm h}{} 31\overset{\rm m}{} 32\overset{{\rm s}}{.}80$ & $+26\overset{\circ}{} 40\overset{\prime}{} 48\overset{{\prime\prime}}{.}18$ & $  70.83$ & $  68.01 \pm  2.04$ &$  12.48$ \\
$11\overset{\rm h}{} 02\overset{\rm m}{} 53\overset{{\rm s}}{.}30$ & $+27\overset{\circ}{} 03\overset{\prime}{} 39\overset{{\prime\prime}}{.}38$ & $  35.19$ & $  28.59 \pm  1.19$ &$  18.43$ &$12\overset{\rm h}{} 50\overset{\rm m}{} 21\overset{{\rm s}}{.}97$ & $+27\overset{\circ}{} 04\overset{\prime}{} 32\overset{{\prime\prime}}{.}95$ & $  49.53$ & $  44.96 \pm  1.43$ &$  18.40$ \\
$09\overset{\rm h}{} 15\overset{\rm m}{} 01\overset{{\rm s}}{.}99$ & $+27\overset{\circ}{} 01\overset{\prime}{} 45\overset{{\prime\prime}}{.}69$ & $  26.15$ & $  30.06 \pm  0.49$ &$  10.34$ & & & & & \\
\hline\hline
\end{tabular}
